Towards Good Practices in Self-supervised Representation Learning

Self-supervised representation learning has seen remarkable progress in the last few years. More recently, contrastive instance learning has shown impressive results compared to its supervised learning counterparts. However, even with the ever increased interest in contrastive instance learning, it is still largely unclear why these methods work so well. In this paper, we aim to unravel some of the mysteries behind their success, which are the good practices. Through an extensive empirical analysis, we hope to not only provide insights but also lay out a set of best practices that led to the success of recent work in self-supervised representation learning.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we dive into the details of recent contrastive instance learning methods and unravel the mysteries behind their success. 
We emphasize that good practices are an integral part of the algorithms.
%For example, MoCo cannot converge without momentum encoder. 
%Performance of SimCLR drops significantly without MLP projection head.
In particular, we investigate on MLP projection head and find that it acts like a filter, separating the information-rich features useful for downstream tasks from the more discriminative feature that are suitable for minimizing the contrastive loss.
We also find that instance discrimination task does not suffer from the semantic label shift problem presented in supervised learning.
Finally, by analyzing both quantity and quality of negative samples, we make an interesting observation that good practices during training eliminate the need of using large number of negatives. 
We hope our empirical evidence can provide insights and better understanding of recent progress, as well as advance future development of self-supervised representation learning.

==> overview.tex <==
\section{Background}
\label{sec:overview}

The goal of contrastive instance learning is to learn representations by distinguishing between similar and dissimilar instances. 
Images are typically perturbed using various augmentation techniques (e.g. random cropping, or color jittering) and a model is trained to map the original images and the perturbed ones as the same latent representation.
It is important to note that in instance discrimination, each image together with its augmented versions is treated as its own class requiring no \textit{a priori} class annotations. 
A generic visual depiction of recent contrastive instance learning methods is shown in Figure \ref{fig:splash_instdisc}. 

\begin{wrapfigure}{r}{0.5\textwidth}
%	\vspace{-7ex}
	\includegraphics[width=7cm]{contrative_learning_v2.png}
%	\vspace{-10ex}
	\caption{A generic visual depiction of recent contrastive instance learning methods.}
	\label{fig:splash_instdisc}
\end{wrapfigure}

More formally, given a set of images $\mathcal{X}$, an image $x$ is uniformly sampled from $\mathcal{X}$ and is augmented using various augmentation techniques $t \in \mathcal{T}$ to generate the positive pairs $x_1^{+}$ and $x_2^{+}$. 
$f_{\theta}$ and $f_{\phi}$ are encoders which map the images to visual representations $h_{1}$ and $h_{2}$, i.e., 2048-dim features from the last average pooling layer of a ResNet \citep{he_cvpr2016_resnet}.
These visual representations are then projected via $g_{\theta}$ and $g_{\phi}$, which are often MLP heads, to lower dimensional features $z_{1}$ and $z_{2}$ for similarity comparison. 
%\textit{n}-MLP heads,
Networks are usually trained by InfoNCE \citep{oord2018representation} loss,
\begin{equation}
\label{eqn:nce}
L_{\text{NCE}} = -\text{log} \frac{\text{exp}[\text{sim} (z_{1}, z_{2})]}{\text{exp}[\text{sim} (z_{1}, z_{2})] + \sum_{i=1}^{K} \text{exp}[\text{sim}(z_{1}, g_{\phi}(f_{\phi}(x_{i}^{-})))]}.
\end{equation}
Here, $\text{sim}(.)$ is the distance metric used to measure the similarity between feature embeddings.
%(e.g., cosine or L2 distance)
$K$ denotes the number of negative examples $x^{-}$ for each $x$ used in computing contrastive loss. 
It has been posited that negative examples are crucial to avoid learning collapsed representations \citep{grill_arxiv2020_byol}, and can be selected from the rest of the dataset $\mathcal{X}$ via different mechanisms, e.g., memory bank \citep{wu_cvpr2018_instdisc}, queue \citep{he_cvpr2020_moco} or large mini-batch \citep{chen_icml2020_simclr}.
By optimizing the objective, the model learns to map similar instances closer and dissimilar instances farther apart in the embedding space. 
For simplicity, we use $f$ and $g$ to denote encoder network and MLP head, $h$ and $z$ to represent the feature before and after MLP head for the rest of the paper. 

%Once the unsupervised pre-training is done, feature $h$ is usually extracted and transferred to  downstream tasks.
In this paper, we mainly use MoCov2 \citep{chen_arxiv2020_mocov2} as an illustrating example, but also include experiments on other methods when needed.
In terms of unsupervised pre-training, we train a ResNet50 backbone for $100$ epochs, unless otherwise stated.
In terms of evaluation, we follow the standard protocol of \citep{wu_cvpr2018_instdisc,he_cvpr2020_moco} to perform linear probe on ImageNet and report top-1 classification accuracy. 
To be specific, we freeze the encoder $f$ and train a supervised linear classifier using feature $h$.
% i.e., a fully-connected layer followed by softmax.
MLP head $g$ is discarded in the evaluation.
%Unsupervised pre-training are trained with ResNet50 backbone for $100$ epochs, unless otherwise stated.
%Take ResNet50 as an example, most literature extract the global average-pooled feature from the last convolutional layer, i.e., $h \in \mathbb{R}^{2048 \times 1}$. 
%There are two standard ways to evaluate the quality of the learned feature embedding: linear probe and end-to-end finetune. 
%For linear probe, we freeze the features $h$ and 
%Usually this is done on ImageNet for fair comparison between methods.
%For end-to-end finetune, the encoder network $f(.)$ is not frozen.
%This is the same as supervised pre-training on a large source dataset then followed by finetuning on a small target dataset.


%Before we dive into answering the aforementioned questions, it is necessary to define the notations and describe the basics of the framework. 
%The criterion for similarity can be defined in many ways. 
%Most literature treat two augmented versions of the same image as similar instance (a.k.a positive example), and all other images as dissimilar instances (a.k.a negative examples).
%Suppose we have a dataset $\mathcal{X}$ and a way to sample positive ($x$, $x^{+}$) and negative pairs ($x$, $x^{-}$), the objective is to minimize the Noise Contrastive Estimation (NCE) loss


%Once the unsupervised pre-training is done, features are extracted typically from the last pooling layer and transferred to a downstream tasks, for example image classification or object detection.
%%Take ResNet50 as an example, most literature extract the global average-pooled feature from the last convolutional layer, i.e., $h \in \mathbb{R}^{2048 \times 1}$. 
%There are two standard ways to evaluate the quality of the learned feature embedding: linear probe and end-to-end finetune. 
%For linear probe, we freeze the features $h$ and train a supervised linear classifier (a fully-connected layer followed by softmax).
%Usually this is done on ImageNet for fair comparison between methods.
%For end-to-end finetune, the encoder network $f(.)$ is not frozen.
%This is the same as supervised pre-training on a large source dataset then followed by finetuning on a small target dataset.

==> related.tex <==
\section{Related Work}
\label{sec:related_work}

\noindent \textbf{Contrastive instance learning}
Instance discrimination is a classification task where each image in a dataset is considered to be in its own class \citep{dosovitskiy_nips2014_exemplar}.
This task can either learn from both positive and negative pairs \citep{wu_cvpr2018_instdisc,he_cvpr2020_moco} or simply learn from positive pairs through consistency \citep{grill_arxiv2020_byol}.
Recently, most work on instance discrimination use contrastive learning to train the network due to its simplicity and effectiveness.
\citet{he_cvpr2020_moco,chen_icml2020_simclr,caron2020unsupervised} have been particularly impressive as these self-supervised models do better than supervised variants \citep{he_cvpr2016_resnet} on downstream tasks.

Interestingly, we find that part of the success of recent self-supervised learning methods actually come from using good practices. 
Inspired by \citep{bachman_nips2019_amdim,cubuk2019autoaugment}, SimCLR \citep{chen_icml2020_simclr} adopts nonlinear projection head and stronger data augmentation to learn better feature representations.
Then, MoCov2 \citep{chen_arxiv2020_mocov2} incorporates these good practices with longer training, and significantly outperform MoCo \citep{he_cvpr2020_moco}.
Followed by this, SimCLRv2 \citep{chen_arxiv2020_simclrv2} uses more MLP heads and momentum encoder in \citet{he_cvpr2020_moco} to again refresh the state-of-the-art. 
Recently, \citet{caron2020unsupervised} show that clustering based representation learning can benefit from aforementioned good practices as well.
Furthermore, consistency based methods like BYOL \citep{grill_arxiv2020_byol} also used MLP head and momentum encoder to achieve promising results, which suggests that these good practices can be generalized beyond contrastive learning paradigm. 

Hence in this work, we deviate from proposing new pretext tasks or new constraints. 
Instead we analyze the effect of good practices in self-supervised learning and unravel the mystery behind the recent success of contrastive instance learning methods.

%There is also a recent work \cite{caron2020unsupervised} that argues neither a
%memory bank nor a momentum encode is necessary for learning effectively from
%instance discrimination.
%%
%It suggests that many recent advances in instance
%discrimination training techniques are quite orthogonal and can be combined
%to achieve better results.



%Recently, most work  
%as a way to circumvent the large number of classes, to learn this task.
%
%In InstDisc \cite{wu_cvpr2018_instdisc}, the authors propose to use memory banks to store previously seen
%instance features.
%%
%In MoCo \cite{he_cvpr2020_moco}, the authors propose a momentum encoder that replaces
%the memory banks and allows them to learn from effectively much larger number of banks.
%%
%In SimCLR \cite{chen_icml2020_simclr}, the authors take another route (different from  \cite{he_cvpr2020_moco}) to
%circumvent the memory banks by use very large batch sizes during training. They also
%show two important network architectural designs that can significantly boost the
%performance of the networks trained using instance discrimination:

%\begin{itemize}
%	\item the use of MLP projection head in both encoder networks
%	\item the use of even stronger single image augmentation than the ones used in
%	both MoCo \cite{he_cvpr2020_moco} and InstDisc \cite{wu_cvpr2018_instdisc}.
%\end{itemize}
%

%In MoCo v2 \cite{chen_arxiv2020_mocov2}, the authors incorporated
%SimCLR \cite{chen_icml2020_simclr}'s projection head and
%stronger augmentation. In SimCLR v2 \cite{chen_arxiv2020_simclrv2},
%the authors incorporated MoCo \cite{he_cvpr2020_moco}'s
%momentum encoder (among other innovations such encoder network distillation). In
%both cases, the authors achieved significantly better performance than
%their previous works.
%

%
%There is also a recent work \cite{caron2020unsupervised} that argues neither a
%memory bank nor a momentum encode is necessary for learning effectively from
%instance discrimination.
%%
%It suggests that many recent advances in instance
%discrimination training techniques are quite orthogonal and can be combined
%to achieve better results.

%to consistently matching the two versions
%of the same image .

%This task is useful in training a network to recoginize if any two images are indeed the same instance. It is
%shown that networks learned in such a fashion are quite good at
%generalizing \cite{zhao2020makes}.

%It is a nontrivial task because 1) the two images could be from the same instance but
%undergo independent yet strong transformations
%such as cropping and color jittering, or 2) the two images could be from different
%instances but actually have similar appearances. This task can either learn from
%both positive and negative sample pairs \cite{wu_cvpr2018_instdisc} or
%simply learn to consistently matching the two versions
%of the same image \cite{grill_arxiv2020_byol}.
%

%
%Dosovitskiy et al. \cite{doersch2015unsupervised} explicitly assigns an individual
%class for each image.
%However, this method would become intractable when we apply it to a large dataset that has millions of images.
%
%

%TODO: all of this moved from introduction to related work. need to better integrate it as related work
\noindent \textbf{Insights and analysis}
With this ever increased interest in contrastive instance learning, there are only few work that shed light on \textit{why} they work so well.
~\citet{wang_arxiv2020_hypersphere} identifies two key properties, alignment and uniformity, related to the contrastive loss and empirically confirms the strong agreement between both metrics and downstream task performance.
~\citet{tian_arxiv2020_goodviews} is a follow-up work of Contrastive Multiview Coding ~\citep{tian2019contrastive} which studies the influence of different view choices in contrastive learning.
Their analysis suggests an ``InfoMin principle'' which inspires a task-dependent representation learning strategy.
~\citet{zhao2020makes} investigates the problem of what makes instance discrimination pre-training good for transfer learning.
Interestingly, they find that the low-/mid-level representations matter the most for object detection transfer, not high-level representations.
~\citet{purushwalkam_arxiv2020_demystify} demystifies the gains from contrastive learning by investigating the invariances encoded in the learned visual representations.
Their results indicate that a large portion of recent gains come from occlusion invariances.
%In order to achieve more invariances like in viewpoint and instance, they propose to use unlabeled video data for contrastive learning.
Recently, \citet{falcon_arxiv2020_yadim} analyze leading SSL approaches and find that despite different motivations, they are special cases under one unified framework.
All aforementioned work provide great insights from different perspectives, while we go with a new one: good practices.
%Our work instead focus on the importance of good practices and show how they contribute to the rapid progress of self-supervised representation learning.

\noindent \textbf{Good practices in deep learning} 
Deep models are known to be sensitive to training techniques. 
A small change in network architecture or learning schedule can significantly impact the final performance.
Numerous good practices have been proposed over the last decade and lead to the current deep learning era.
The great success of AlexNet \citep{krizhevsky_nips2012_alexnet} benefits from using color augmentation, Dropout layer and ReLU activation. 
\citet{gulrajani_nips2017_improvedWGAN} stabilizes the training of generative adversarial networks (GAN) by introducing gradient penalty, and makes GAN accessible to more people. 
\citet{he_cvpr2019_bagoftricks} ensembles multiple training procedure refinements in image classification, like learning rate warmup, no bias decay, label smoothing, etc., so that stronger backbones can be trained and transferred to downstream tasks.
Similarly, \citet{bochkovskiy_arxiv2020_yolov4} combines good practices in object detection over the years and builds a more accurate and faster object detector YOLOv4.
Hence, good practices are important, sometimes even essential, for deep network learning. 
Furthermore, it is also beneficial to understand how they work, which could be inspiration for further improvement. 

%Putting the progress in contrastive learning aside for a moment, many recent results also seem to contradict what we have known in supervised learning.
%For example,~\citep{bachman_nips2019_amdim,chen_icml2020_simclr} have shown that simply adding a nonlinear projection head between the last pooled convolutional feature and the final classification layer can significantly improve the quality of learned representations.
%Quantitatively, the nonlinear projection head can help to improve top-1 classification accuracy on ImageNet by over $10\%$ in~\citet{chen_icml2020_simclr} and $5.6\%$ in~\citet{chen_arxiv2020_mocov2}.
%However, adding such a shallow multilayer percepton (MLP) projection head (i.e., one fully-connected layer and one activation layer) is often not effective in supervised learning.
%Take another example, recent methods such as~\citep{he_cvpr2020_moco,chen_icml2020_simclr} adopt aggressive and strong data augmentation during contrastive pre-training. 
%Although data augmentation has been proven to be useful, overly aggressive augmentations often lead to worse results in supervised or other self-supervised learning methods.
%Then why can contrastive learning  benefit from strong data augmentation?
%Furthermore, contrastive learning based on instance discrimination usually requires a large number of negative examples when computing contrastive loss.
%Because of this, researchers design various mechanisms to store the negative examples, such as memory bank \cite{wu_cvpr2018_instdisc,misra2020self}, queue \cite{he_cvpr2020_moco,chen_arxiv2020_mocov2} or simply large mini-batch \cite{chen_icml2020_simclr,chen_arxiv2020_simclrv2}.
%But is it really necessary?
%At this moment and to the best of our knowledge, there is no concrete evidence to answer these questions.




%\subsection{Distance Metric Learning}
%%TBA \cite{ji2019invariant} \cite{caron2018deep}
%
%% One could consider deep metric as the supervised 
%
%Similar to instance discrimination, deep metric learning also aims to learn a representation of input images, but in a supervised fashion with explicit class labels. Early works considered pairwise losses of pairs~\cite{contrastiveloss} and triplets~\cite{tripletloss} with the aim of minimizing the distance between the instances of the same class (anchor and positive) while maximizing the distance to the instance of another class (negative). Formally, the triplet loss is expressed as
%
%\begin{equation}
%	L_{triplet} = |d_{ap} - d_{an} +m|_{+}
%\end{equation}
%
%where $m$ is a predefined margin. The distance function is typically defined as the Euclidean or cosine distance. Recent years many metric learning losses were proposed on top of the triplet principle. For example, ~\cite{wang2017deep} considers the angles between triplet vectors to establish the margins, while~\cite{wu2017sampling} extends the fixed margin with a learnable additive coefficient. One core challenge of these losses is the composition of triplets. In fact while selecting all possible triplets in a dataset is typically intractable, choosing only the "easy" ones will provide zero loss, while too "hard" ones could lead to the collapse of the latent space. Initially, offline mining for the best triplet candidates have been proposed via storing a list~\cite{minding_list}, or using a nearest neighbor search before each epoch~\cite{smartmining}. A more efficient semi-hard negative mining method for each mini-batch was presented by~\cite{schroff2015facenet}. Later~\cite{wu2017sampling} found that distance weighted sampling improves the diversity of the negative samples in the batch, thus improving the performance.
%
%Classification-based losses were also proposed for metric learning~\cite{wang2017normface, normproxies} that probably resemble the most to contrastive learning. In fact, these approaches consider L2 normalized embeddings multiplied with a learned weight matrix to obtain the logits. Margins have also been considered as additive-cosine~\cite{wang2018additive}, additive-angular~\cite{Deng_2019_CVPR}, or multiplicative-angular~\cite{sphereface}.

%\subsection{Augmentation and pretext tasks}
%
%Many recent advances in self-supervised learning benefit from strong
%augmentation and various pretext tasks \cite{misra2020self,doersch2017multi}. Instance discrimination
%is one type of pretext tasks.
%Other popular pretext tasks include colorization \cite{zhang2016colorful},
%in-painting \cite{pathak2016context}, learning to count \cite{noroozi2017representation},
%learning from motion \cite{agrawal2015learning},
%solving jigsaw puzzles \cite{noroozi2016unsupervised},
%rotation \cite{gidaris2018unsupervised},
%multi-view/channel \cite{tian_arxiv2020_goodviews, zhang2017split, bachman_nips2019_amdim, tian2019contrastive}
%learn to generate \cite{donahue2016adversarial}, etc.
%
%Recent works seem to suggest that a simple pretext task (e.g., instance discrimination)
% paired with strong, sophisticated image augmentation can sometimes achieve better results
% than the ones that rely on sophisticated pretext
% tasks \cite{tian2019contrastive,oord2018representation,chen_arxiv2020_mocov2,caron2020unsupervised}.
% We also notice that the aggressive augmentation transformations used in
%  \cite{wu_cvpr2018_instdisc} (and works following it) would typically have
% adverse effect if used in supervised setting.
%
%Therefore, it is interesting for us to know why strong data augmention is
%so beneficial for self-supervised learning.

